HeteGCN: Heterogeneous Graph Convolutional Networks for Text Classification

We consider the problem of learning efficient and inductive graph convolutional networks for text classification with a large number of examples and features. Existing state-of-the-art graph embedding based methods such as predictive text embedding (PTE) and TextGCN have shortcomings in terms of predictive performance, scalability and inductive capability. To address these limitations, we propose a heterogeneous graph convolutional network (HeteGCN) modeling approach that unites the best aspects of PTE and TextGCN together. The main idea is to learn feature embeddings and derive document embeddings using a HeteGCN architecture with different graphs used across layers. We simplify TextGCN by dissecting into several HeteGCN models which (a) helps to study the usefulness of individual models and (b) offers flexibility in fusing learned embeddings from different models. In effect, the number of model parameters is reduced significantly, enabling faster training and improving performance in small labeled training set scenario. Our detailed experimental studies demonstrate the efficacy of the proposed approach.

==> sections/Formulation.tex <==
\section{Motivation and Problem Formulation} 

\textbf{Problem Formulation.} We are given a document corpus ($\bfx)$ with a set of labeled and  unlabeled examples. Additionally, we may have access to $\bff$. Our goal is to learn feature embeddings ($\bfu$) using simple and efficient graph convolutional networks and learn an inductive classifier model to predict the target class.  

==> sections/background.tex <==
\section{Preliminaries}
\label{sec:preliminaries}
\subsection{Notation}
In this section, we introduce notation used throughout the paper. We use $x_i \in {\mathcal R}^m$ to denote $m$-dimensional feature vector of $i^{th}$ example, $y_i \in \{1,\ldots,k\}$ to denote the corresponding binary representation of target class and $k$ to denote the number of classes. We use $\bfx$ to denote the \textit{document-feature} matrix of the entire corpus (where each row represents the feature vector of an example) and $\mathcal{L}_{tr}$ to denote the set of labeled training examples. We use $\bff$ to denote a \textit{feature-feature} relation matrix and $\bfn$ to denote a \textit{document-document} relation matrix. The relation matrices are either explicitly provided or implicitly constructed from $\bfx$. We view each matrix as a graph (and vice-versa) with rows and columns representing nodes. For example, $\bfx$ is a bipartite graph connecting document nodes and feature nodes with edge weights that may be set to \textsc{TF-IDF} scores. We use $\bfsv_i = Emb(d_i)$ ($i \in \{1,\ldots,n\}$) to denote the document embedding of the $i^{th}$ document and $\bfsu_j = Emb(f_j)$ to denote the embedding of the $j^{th}$ feature ($j \in \{1,\ldots,m\}$). The corresponding embedding matrices are denoted as $\bfv$ and $\bfu$ respectively. Finally, $\bfi_n$ and $\bfw$ denote the $n$ dimensional identity matrix and the network model weights respectively. We use $\bfp$ to denote the class probability distribution of documents over $k$ classes. In this paper, the terms \textit{document} and \textit{example} are used interchangeably. Similarly, we use \textit{feature} and \textit{word} interchangeably. Note that in some privacy sensitive applications, \textit{words} are not available and only hashed feature identifiers are available. 

%For example, [TextGCN] constructs $F$, a point-wise mutual information (PMI) matrix from the raw text data using words (features) available in a fixed length neighborhood window. Similarly, [GCN] assumes that a link graph $N$ encoding relational information between documents is given. When relational graphs are not directly available they are often derived from $\bfx$ as: $\bff = \bfx^T \bfx$ and $\bfn = \bfx \bfx^T$ after some pre-processing (e.g., normalization) and post-processing (e.g., selecting a few nearest neighbors) steps. 

%We view each matrix as a bipartite graph (and vice-versa) with rows and columns representing nodes, and edges connecting nodes with non-zero matrix entries. For example, $\bfx$ is a bipartite graph connecting document nodes and feature nodes with edge weights that may be set to \textsc{TF-IDF} scores. This graph is heterogeneous as it connects entities of different types (i.e., \textit{document} and \textit{feature}). Similarly, $\bff$ and $\bfn$ are homogeneous graphs connecting feature nodes and document nodes respectively. 

 \subsection{Background}
  %In this section, we briefly present several important graph embedding models and methods that motivated our work. 
 \textbf{Predictive Text Embedding (\pte).} Tang et al.~\cite{pte} proposed a semi-supervised embedding learning method that makes use of both labeled and unlabeled documents. They construct a heterogeneous text graph which is a composition of three graphs, document-word ($\bfx$), word-word ($\bff$) and word-label ($\bfl$). Note that $\bfx$ and $\bff$ are available for the entire corpus and $\bfl$ is constructed using only labeled training examples. The core idea is to learn \textit{shared} word embeddings ($\bfu$) by leveraging labeled information available through $\bfl$ jointly with $\bfx$ and $\bff$. 
 %Embeddings are learned using efficient \textsc{LINE} (Large scale Information Network Embedding) modeling approach. 
 The embedding of any document is computed as an average of the embeddings of words present in the document. Finally, a linear (\textsc{Softmax}) classifier model is learned by minimizing cross-entropy loss function with labeled training examples: 
 \begin{equation}
 {\mathcal M}(\bfw) = \sum_{i \in {\mathcal L}_{tr}} \sum_{k} y_{i,k} \ln(p(y_{i,k}|\bfsv_i;\bfw))
 \label{eqn:training}
 \end{equation}
 Note that the embeddings and classifier model are learned \textit{sequentially}. \pte is efficient and has inductive capability. 
 
 \textbf{Graph Convolutional Network .} Kipf et al.~\cite{gcn} proposed a semi-supervised learning method using graph convolutional networks. A graph convolutional network is a multi-layer network and each layer takes node embeddings ($\bfe^{(l)})$ of the $l^{th}$ layer as input and produces either embeddings ($\bfe^{(l+1)})$ for the $(l+1)^{th}$ layer or predictions for a given task (e.g., target class probability distribution) at the final layer. Formally, $\bfe^{(l+1)} = g(\bfa,\bfe^{(l)},\bfw^{(l)})$ where $\bfe^{(l)}$ and $\bfw^{(l)}$ denote the embedding and weight matrices of the $l^{th}$ layer respectively. $g(\cdot)$ is a transformation function (e.g., \textsc{ReLU} or \textsc{Softmax}), and $\bfe^{(0)}$ is the input feature matrix (e.g., $\bfx$) or 1-hot encoding representation of nodes (i.e., $\bfi_n$). $\bfa$ denotes an adjacency matrix and is fixed across layers. Like \pte, the model weights $\bfw$ are learned using only labeled training examples using (\ref{eqn:training}). However, \gcn is only transductive, as embeddings for unseen documents cannot be computed during inference. 
 %\gcn assumes that a link graph $\bfn$ encoding relational information between documents is given. When $\bfn$ is not available, a $l$-nearest neighbor graph is constructed from $\bfx$ using some distance function (e.g., Cosine Similarity). Like \textsc{PTE}, the model weights $\bfw$ are learned using only labeled training examples. However, \textsc{GCN} is only transductive as embeddings for unseen documents cannot be computed during inference.            
 
 \textbf{TextGCN}. Yao et al.\cite{textgcn} proposed a text graph convolutional network (\textsc{TextGCN}) method by using the matrix: 
 \begin{equation}
 \bfa = \begin{bmatrix}
 \bff & \bfx^T \\
 \bfx & {\bf 0}
 \end{bmatrix}
 \label{eqn:A}
\end{equation}
in \textsc{GCN} across layers. Note that it makes use of both \textit{word-word} and \textit{document-word} relational graphs excluding $\bfn$ (which may not be explicitly available). With a two-layer network, document-document relations are inferred and used along with word embeddings to obtain document embeddings. \textsc{TextGCN}~\cite{textgcn} achieved significantly improved accuracy performance over \pte. It is important to note that \tgcn does not make use of $\bfl$ and the gain mainly comes from using \gcn architecture. Nevertheless, \tgcn has several limitations which we explain next. 

Consider the first layer output of \tgcn. With $\bfa$ as given in~\ref{eqn:A}, the feature and document embedding matrices are given by: 
{\small
\begin{align}
    \bfu^{(1)} = g(\bff \bfi_m \bfw_u^{(0)} + \bfx^T \bfi_n \bfw_v^{(0)}), \bfu^{(2)} = g((\bff \bfu^{(1)} + \bfx^T \bfv^{(1)}) \bfw_u^{(1)}) \label{eqn:wemb} \\ 
    \bfv^{(1)} = g(\bfx^T \bfi_n \bfw_v{(0)}), \bfp = \textsc{Softmax}(\bfx \bfu^{(1)} \bfw_v^{(1)}) \label{eqn:demb}
\end{align}
}
where 1-hot representation is used for features and documents. The subscripts used in $\bfw_v^{(0)}$ and $\bfw_u^{(0)}$ denote the embedding type in the first (\textit{aka} input) layer. In other layers, we use the subscript in the weight matrix (e.g., $\bfw_v^{(1)}$) to match the type of multiplicand.   
%Note that the document embedding matrix used by the \textsc{Softmax} classifier model is given by: 
%\begin{equation}
%    \bfu^{(2)} = \bfx \bfv^{(1)} = \bfx g(\bff \bfi_m \bfw_v^{(0)} + \bfx^T \bfi_n \bfw_u^{(0)}).  
%\end{equation}
%We make several important observations: (1) the feature embeddings are computed using both $\bfw_v^{(0)}$ and $\bfw_u{(0)}$, 

We make two important observations. The number of model parameters is dependent on the number of features ($m$) and documents ($n$). This implies \tgcn is not suitable for large scale applications when $(n+m)$ is very large with $n \gg m$. Furthermore, when the number of labeled training examples is small it is difficult to learn large number of model parameters reliably, resulting in poor generalization. Next, learning document embedding using (\ref{eqn:A}) makes \tgcn transductive. 

Motivated by the success of \textsc{PTE} and \textsc{TextGCN} in semi-supervised text classification, yet recognizing their limitations, our interest lies in designing a graph convolutional network based approach that brings the best capabilities of \textsc{PTE} (i.e., efficient training and inductive) and \textsc{TextGCN} (i.e., superior performance) together.  

\textbf{Problem Formulation.} We are given a document corpus ($\bfx)$ with a set of labeled and unlabeled examples. Additionally, we may have access to $\bff$ and $\bfn$. Our goal is to learn feature embeddings ($\bfv$) using simple and efficient graph convolutional networks and learn an inductive classifier model that makes use of document embedding computed using $\bfv$ to predict the target class.  
 
 
